On the inductive biases of deep domain adaptation

Domain alignment is currently the most prevalent solution to unsupervised domain-adaptation tasks and are often being presented as minimizers of some theoretical upper-bounds on risk in the target domain. However, further works revealed severe inadequacies between theory and practice: we consolidate this analysis and confirm that imposing domain invariance on features is neither necessary nor sufficient to obtain low target risk. We instead argue that successful deep domain adaptation rely largely on hidden inductive biases found in the common practice, such as model pre-training or design of encoder architecture. We perform various ablation experiments on popular benchmarks and our own synthetic transfers to illustrate their role in prototypical situations. To conclude our analysis, we propose to meta-learn parametric inductive biases to solve specific transfers and show their superior performance over handcrafted heuristics.

==> bounds.tex <==
%\section{Learning Bounds and relation to domain-adversarial training}
\section{Can generalization bounds help to build good alignment methods?}\label{sec:theory}

In this section, we start by defining some notations, then we give the main generalisation bounds of the literature. We then explain why these bounds do not explain the results obtained in domain adaptation.

We call \textit{source} and \textit{target} domains two distributions $S$ and $T$ over the space of labeled data $X\times Y$. We define $S_X$ and $T_X$ the marginals of $S$ and $T$ over $X$ and $S_Y$, $T_Y$ the marginals over $Y$. Finally, we call \textit{domain shift} the discrepancy existing between $S$ and $T$. We study \textit{unsupervised domain adaptation}: provided labeled samples from $S$ and unlabeled samples from $T$, we would like to exploit labeled knowledge from $S$ to obtain a model that minimizes the target risk.

Obviously, this can only be possible if a relationship between $S$ and $T$ exists. The following general cases are often described in the literature: i)  \textem{Covariate shift / inductive transfer}: $S_X \neq T_X$ and $P_S(Y | X) = P_T(Y | X)$ ii)  \textem{Concept shift / transductive transfer}: $S_X = T_X$ and $P_S(Y | X) \neq P_T(Y | X)$
    iii)  \textem{Unsupervised transfer}: $S_X \neq T_X$ and $P_S(Y | X) \neq P_T(Y | X)$.

When doing transfer learning with deep networks, we expect the labeling function to be consistent across domains and only account for qualitative shifts in input data distribution, we hence focus on the covariate shift problem. 
\subsection{Learning Bounds:}
 The majority of bounds proposed in the literature take the form of upper bounds on the risk in the target domain. Given the extent of the literature and the profusion of these bounds, we only detail those that have been used to justify  domain alignment algorithms. We strongly encourage the reader to refer to \cite{SurveyDomainAdaptationTheory} for an exhaustive analysis of other existing bounds.

\textbf{The seminal Ben-David bound:} Let $\mathcal{H}$ be our hypothesis space. We define the expected 0-1 risk $\epsilon_D(h,  f)$ of an hypothesis $h\in \mathcal{H}$ on a domain $D$ labeled by $f$. We abuse the notation slightly to write the expected disagreement on $D$ between two hypotheses as $\epsilon_D(h, h')$.\\
In unsupervised domain adaptation, the goal is to find some $h$ that minimizes the target risk $\epsilon_T(h,  f)$, provided labels from $S$.
As the objective is to control the target error, we seek an informative upper bound on this quantity that we can minimize. The first result of this type was provided by \cite{bendavid}. They propose the following bound, valid in the covariate shift assumption, e.g. $f_S = f_T = f$:
\begin{center}
\begin{equation}
    \begin{split}
        \epsilon_T(h,f)\leq&\epsilon_S(h,f)+\lambda +\delta_{H\Delta H}(S_X,T_X)
    \end{split}
    \label{eq:bendavid}
\end{equation}   
\end{center}

where, $\lambda:=\inf_{h'} \epsilon_S(h', f)+\epsilon_T(h', f)$ is the optimal combined error on source and target, and
$\delta_{H\Delta H}(S_X,T_X):=\sup_{h,h'\in H}\epsilon_T(h,h')-\epsilon_S(h,h')$ is called the $H\Delta H$-divergence, and accounts for how much two
hypotheses can deviate from one another and in a different way in the two domains. This quantity can be interpreted as an hypothesis-dependent discrepancy between probability densities.\\

\textbf{Zhang et al. bound:}
By removing a supremum over $h$ during the bound computation, \cite{mdd} further refined the bound by relaxing the divergence to a single adversarial hypothesis:
\begin{center}
\begin{equation}
    \begin{split}
        \epsilon_T(h,f)\leq&\epsilon_S(h,f)+\lambda +\delta_{h, H}(S_X,T_X)
    \end{split}
    \label{eq:zhang}
\end{equation}  
\end{center}

where $\delta_{h, H}(S_X,T_X):=\sup_{h'\in H}\epsilon_T(h,h')-\epsilon_S(h,h')$. This bound is strictly tighter than Ben David's and improves on the fact that $\delta_{h, H}$ can be evaluated through adversarial training (taking $h'$ as adversarial hypothesis), then minimized w.r.t. $h$, hence "Bridging Theory and Algorithm".\\ 


\textbf{Wasserstein bound:}\cite{WassersteinDAShen2017} proposed a domain adaptation upper-bound that builds on the Wasserstein distance, a popular framework that exploits the underlying base L1-metric between samples to give a smooth measure of discrepancy between non-overlapping distributions. Due to the change of framework, we use metric-based errors in this bound. It applies under the assumption that the hypothesis class is restricted to $K$-Lipschitz functions, which is not an issue as the Lipschitz constant of deep models can be controlled with regularization {\color{red} (normalization rather ?)} \cite{SpectralNorm}.

\begin{equation}
    \begin{split}
        \epsilon^{L1}_T(h)\leq&\epsilon^{L1}_S(h)+\lambda + 2KW_1(S_X,T_X)
    \end{split}
    \label{eq:wasserstein}
\end{equation}

With $\epsilon^{L1}_D(h)$ the L1 classification cost on domain D and $\lambda$ the joint L1 error of the best hypothesis and $K$ the Lipschitz constant of the hypothesis class.

Many other bounds were proposed until now, but all of them have a shape similar to those presented, and mainly differ on the divergence used to compare source and target marginal distributions.

\subsection{Link between minimization of these bounds and domain adaptation algorithms}

In order to derive a domain adaptation method from these bounds, one has to find a way to minimize them. In any case, the error term of the in the source domain can be directly controlled by the supervision available on the source, and the term $\lambda$ is assumed to be zero when choosing a sufficiently expressive $\mathcal{H}$. 

In realistic computer vision problems, we have to take into account the fact that $supp(S_X)\cap supp(T_X)=\emptyset$.  For example, if the domains are, on the one hand, images of objects and, on the other hand, drawings of these objects, no image from one domain can exist in the other domain. 
Having non-overlapping domains is likely to make all divergence terms used in the bounds maximal. Indeed, divergence used in bounds \ref{eq:bendavid} and \ref{eq:zhang} depends on the capacity of a chosen hypothesis family to discriminate source and target samples. Even with simple linear models, these discrepancies can reach prohibitively high values, making the bounds helpless when high-capacity deep models are used, assuming fixed $S_X$, $T_X$. To circumvent this problem, using optimal transport distances such as Wasserstein-1 instead of hypothesis-based distances might be appealing: optimal transport exploits the underlying space metric to build new discrepancies that are smooth and informative when supports do not overlap. However, we can prove that bound \ref{eq:wasserstein} is equally uninformative in the general case:

We would like to optimize bound \ref{eq:wasserstein} w.r.t. $K$, which is impossible in the general case as we cannot evaluate $\lambda$: If $K$ is too small, then the hypothesis class is too smooth and cannot achieve good joint L1-error on both domains (e.g. high $\lambda$ and $\epsilon^{L1}_S(h)$). If it is too large, so does the discrepancy term. We provide an illustration of the overall trade-off in figures [les .png ne chargent pas].

With fixed $S_X$ and $T_X$, it is not possible to minimize such bounds as there is an uncompressible trade-off between model expressivity and domain-invariance.
The idea of domain-alignment methods is to replace $S_X$ and $T_X$ by representation vectors outputted by a representation network $\Psi$, trained to minimize the discrepancy between $S_X$ and $T_X$ while ensuring good source accuracy by a subsequent classifier $h$. Citing bound \ref{eq:bendavid} as its reference, DANN \cite{dann} uses adversarial training to minimize distributions and hence minimizes the Jensen-Shannon divergence as a proxy for $H\Delta H$. Using bound \ref{eq:zhang}, MDD \cite{mdd} minimizes $\delta_{h, H}$ by training an adversarial classifier. Finally, WDGRL \cite{WassersteinDAShen2017} minimizes the wasserstein distance of bound \ref{eq:wasserstein} using the WGAN-GP framework \cite{wgangp}.\\
In each of those cases, this practice is flawed for the same reason: $\Psi$ being non-invertible, aligning marginals  might superpose samples with different labels, breaking the covariate shift assumption and guarantee of having a small $\lambda$.\\ 

Failure of domain-alignment methods reveals the no-free-lunch aspect of those bounds: they do not give a principled minimization algorithm, as minimization of the different terms are not independent problems.




==> theory_old.tex <==
\section{Domain Adaptation Theory}\label{sec:theory}
Many contributions were proposed to better frame the theoretical insights of the domain adaptation problem. They aim at 1) finding informative upper bounds on target risk to estimate the transferability of a classification task between two domains and 2) studying their hardness.\\ Such bounds typically depend on a measure of discrepancy between source and target marginal distributions and complexity of the chosen hypothesis space, and were used as an inspiration to derive practical domain adaptation methods for deep learning. In this paper, we first show that all bounds proposed give trivial, uninformative results in the context of deep vision problems and hence cannot explain alone the experimental success of deep domain adaptation methods. To fill this gap, we analyze the inductive biases found in optimization of pre-trained models (an ubiquitous practice in the literature) and show that they might be the principal ingredients of success when adapting domains.\\
In this section, we will carefully describe the domain adaptation problem. We start from the general case and then increase our focus on the deep vision case. Finally, we confront well-known domain adaptation bounds to this setting and prove their unusefulness.

\subsection{Formalism and definitions}

Let $S$, or \textit{source domain}, be a distribution over the space of labeled data $X\times Y$. Let $T$, or \textit{target domain}, be another data distribution. We define $S_X$ and $T_X$ the marginals of $S$ and $T$ over $X$ and $S_Y$, $T_Y$ the marginals over $Y$.\\
Finally, we call \textit{domain shift} the discrepancy existing between $S$ and $T$.\\ 

Obviously, we expect $S$ and $T$ to be somehow related. To account for this, a taxonomy of domain shifts must be established. The following learning settings are often described in the literature:
\begin{itemize}
    \item \textbf{Covariate shift / inductive transfer}: \\$S_X \neq T_X$ and $P_S(Y | X) = P_T(Y | X)$
    \item \textbf{Concept shift / transductive transfer}: \\$S_X = T_X$ and $P_S(Y | X) \neq P_T(Y | X)$
    \item \textbf{Unsupervised transfer}: \\$S_X \neq T_X$ and $P_S(Y | X) \neq P_T(Y | X)$
\end{itemize}
When doing transfer learning with deep networks, we solve a problem of the first category. Until the end of the paper, we will hence focus on the covariate shift problem. Indeed, in transfer learning, we expect the labeling function to be consistent across domains and only account for qualitative shifts in input data distribution.

\subsection{Usefulness of domain adaptation bounds in deep vision}
Let $\mathcal{H}$ be our hypothesis space. We define the expected 0-1 risk $\epsilon_D(h,  f)$ of an hypothesis $h\in \mathcal{H}$ on a domain $D$ labelled by $f$. We abuse the notation slightly to write the expected disagreement on $D$ between two hypotheses as $\epsilon_D(h, h')$.\\
In unsupervised domain adaptation, the goal is to find some $h$ that minimizes the target risk $\epsilon_T(h,  f)$, provided labels from $S$.
As the objective is to control the target error, we seek an informative upper bound on this quantity that we could minimize. The first result of this type was provided by \cite{bendavid}. They propose the following bound, valid in the covariate shift assumption, e.g. $f_S = f_T = f$:
\begin{center}
\begin{equation}
    \begin{split}
        \epsilon_T(h,f)\leq&\epsilon_S(h,f)+\lambda +\delta_{H\Delta H}(S_X,T_X)
    \end{split}
\end{equation}   
\end{center}

where, $\lambda:=\inf_{h'} \epsilon_S(h', f)+\epsilon_T(h', f)$ is the optimal combined error on source and target, and
$\delta_{H\Delta H}(S_X,T_X):=\sup_{h,h'\in H}\epsilon_T(h,h')-\epsilon_S(h,h')$ is called the $H\Delta H$-divergence, and accounts for how much two
hypotheses can deviate from one another and in a different way in the two domains.\\\\
\cite{mdd} further refined the bound by relaxing the divergence to a single adversarial hypothesis:
\begin{center}
\begin{equation}
    \begin{split}
        \epsilon_T(h,f)\leq&\epsilon_S(h,f)+\lambda +\delta_{h, H}(S_X,T_X)
    \end{split}
\end{equation}  
\end{center}




where $\delta_{h, H}(S_X,T_X):=\sup_{h'\in H}\epsilon_T(h,h')-\epsilon_S(h,h')$

\cite{mansour} proposed another hypothesis-dependent bound that does not involve any $\lambda$ and generalizes to non-covariate shifts ($f_S\neq f_T$):

\begin{center}
 \begin{equation}
    \begin{split}
        \epsilon_T(h,f_T)-\epsilon_T(h^{*}_T,f_T)\leq\epsilon_S(h, h^{*}_S)+\delta(S_X, T_X)+\epsilon_S(h^{*}_T, h^{*}_S)
    \end{split}
\end{equation}   
\end{center}


Note that all these quantities can be estimated from finite samples, but when doing so we must account for an an additional generalization error term that depends on the complexity of the hypothesis space, expressed either with VC, Rademacher or PAC-Bayes frameworks. Deep learning models are overparametrized and hence have very high complexity. However, 1) gradient descent training benefits to generalization in a way that is not entirely understood and 2) those models can be regularized by L1, L2 penalties or dropout, which helps obtaining the model that fits the data with the lowest possible complexity. For those reasons, we think that estimating empirical quantities is not a fundamental issue in domain adaptation theory.

Many other bounds were proposed until now, but all of them have a shape similar to those presented, and mainly differ on the divergence used to compare source and target marginal distributions.
\cite{SurveyDomainAdaptationTheory} gathered an exhaustive listing of these results.

In realistic computer vision problems, we must account for the fact that $supp(S_X)\cap supp(T_X)=\emptyset$. (you may want to adapt a model from daytime imagery to nighttime imagery, but a day image has zero probability of the distribution of night images and vice-versa). In this case, comparing conditionals $P_S(Y|X)$ and $P_T(Y|X)$ is not possible anymore, as we cannot condition on the null event. The mathematical description of covariate shift is therefore obsolete, we replace it by the loose assumption that "images from both domains contain the same classes".\\
Having non-overlapping domains is likely to make all discrepancy terms used in the bounds maximal. Indeed, those quantities ($H\Delta H$ divergences, S-discrepancies, Integral probability metrics...) depend on the capacity of a chosen hypothesis family to discriminate source and target samples. Even with simple linear models, these discrepancies can reach high values, making the bounds helpless when deep models are used.\\

To circumvent this problem, using optimal transport distances such as Wasserstein-1 instead of hypothesis-based distances might be appealing. Optimal transport exploits the underlying space metric to build new discrepancies that are robust to non-overlap of supports.\\
\cite{WassersteinDAShen2017} proposed a domain adaptation upper-bound that builds on the Wasserstein distance. It applies under the assumption that the hypothesis class is restricted to $K$-Lipschitz functions, which is not an issue as the Lipschitz constant of deep models can be controlled with regularization \cite{SpectralNorm}.  


\begin{equation}
    \begin{split}
        \epsilon^{L1}_T(h)\leq&\epsilon^{L1}_S(h)+\lambda + 2KW_1(S_X,T_X)
    \end{split}
\end{equation}

With $\epsilon^{L1}_D(h)$ the L1 classification cost on domain D and $\lambda$ the joint error of the best hypothesis and $K$ the Lipschitz constant of the hypothesis class.\\
We would like to optimize the bound w.r.t. $K$, which is impossible in the general case as we cannot evaluate $\lambda$: If $K$ is too small, then the hypothesis class is too smooth and cannot achieve good joint L1-error on both domains (e.g. high $\lambda$). If it is too large, so does the discrepancy term.\\
We provide an illustration of the overall trade-off in figures 1-2.

\begin{figure}
    \centering
    \includegraphics[scale=0.3]{good_lip.png}
    \caption{Easy case for the Wasserstein bound: an hypothesis class with low K and $\lambda$ exists and Wasserstein distance between domains is low}
    \label{fig:my_label}
\end{figure}

\begin{figure}
    \centering
    \includegraphics{bad_lip.png}
    \caption{Class mixup case: Wasserstein distance between domains is low, but only hypothesis classes with very high K have low $\lambda$. The bound is therefore useless.}
    \label{fig:my_label}
\end{figure}

To derive a domain adaptation method from those bounds, one must find a way to minimize them. The source error term can be easily controlled by the available supervision on source, and the $\lambda$ term is assumed to be null when choosing a sufficiently expressive $\mathcal{H}$. The discrepancy term, however, can only be minimized w.r.t. $S_X$ and $T_X$. The idea of minimizing the discrepancy inspired a wide family of deep domain alignment methods [].\\
To make this possible, we replace $S_X$ and $T_X$ by feature vectors outputed by a representation network.  Working on a feature space is a common practice when dealing with complex data. In deep computer vision, for example, the feature space will be the output of some large network, usually pre-trained on a vast 3-rd party dataset such as ImageNet. However, we make the following observations:
 \begin{itemize}
     \item Pre-trained feature spaces are robust: even on downstream datasets, without any fine-tuning, descriptors are more likely to cluster w.r.t. image class. However, the potential non-invertibility of the feature extractor \cite{johansson2019support} renders the labelling function less deterministic, which involves an increase of the Bayes risk, especially on downstream domains and classes.
     
     \item Distributions of pre-trained features obtained by encoding two domains usually have disjoint supports. However, in many cases, they can be related to each other w.r.t. other metrics.
     
 \end{itemize}
 Therefore, using frozen features as new $S_X$ and $T_X$ does not improve the bounds.
 A lot of authors hence choose to fine-tune the feature-extractor to solve both problems. Alignment of features can be done by minimizing a differentiable discrepancy or by adversarial training. The key point is that this practice violates the theory, aligning marginals might superpose samples from different labels: if we reason with bounds 1, 2 and 4, we break up the (once reasonable) assumption that $\lambda$ is small. With bound 3, it is the term $\epsilon_S(h^{*}_T, h^{*}_S)$ that gets out of control.
 

